Conductors of wild extensions of local fields, especially in mixed characteristic (0,2)

If K_0 is the fraction field of the Witt vectors over an algebraically closed field k of characteristic p, we calculate upper bounds on the conductor of higher ramification for (the Galois closure of) extensions K_0(zeta_{p^r}, sqrt[p^r]{a})/K_0, where a is in K_0(zeta_{p^r}). Here zeta_{p^r} is a primitive p^r-th root of unity. In certain cases, including when a is in K_0 and p=2, we calculate the conductor exactly. These calculations can be used to determine the discriminants of various extensions of Q obtained by adjoining roots of unity and radicals.

==> usuals.tex <==
\def\ints{{\mathbb Z}}
\def\rats{{\mathbb Q}}
\def\nats{{\mathbb N}}
\def\reals{{\mathbb R}}
\def\complex{{\mathbb C}}
\def\quats{{\mathbb H}}
\def\proj{{\mathbb P}}
\def\aff{{\mathbb A}}
\def\FF{{\mathbb F}}
\def\Gp{{\mathbb G}}
\def\adeles{{\mathbb A}}
\def\Ab{{\mathfrak Ab}}
\def\Hecke{{\cal H}}
\def\Fourier{{\cal F}}
\def\one{{\bf 1}}
\def\diag{{\bf diag}}
\def\del{{\partial}}
\def\Span{{\textsc Span}}
%\def\qed{\begin{flushright} $\Box$ \end{flushright}}
\def\qed{\hfill $\Box$}
\def\Im{{\text{Im }}}
\def\im{{\text{im }}}
\def\lcm{{\text{lcm }}}
\def\rank{{\text{rank }}}
\def\sech{{\text{sech }}}
\def\csch{{\text{csch }}}
\def\st{{\text{ s.t. }}} 
\def\nullity{{\text{nullity }}}
\def\Re{{\text{Re}}}
\def\Hom{{\text{Hom}}}
\def\sheafhom{\mathcal{H}om}
\def\Tor{{\text{Tor}}}
\def\cd{{\text{cd }}}
\def\ord{{\text{ord}}}
\def\trace{{\text{tr }}}
\DeclareMathOperator{\eff}{eff}
\def\res{{\text{res}}}
\def\Proj{{\text{Proj }}}
\def\Hess{{\text{Hess }}}
\def\grad{{\text{grad }}}
\def\cf{{\text{char}}}
\def\Frac{{\text{Frac}}}
\def\codim{{\text{codim }}}
\def\coker{{\text{coker }}}
\def\height{{\text{ht }}}
\def\Ext{{\text{Ext}}}
\def\trdeg{{\text{tr.deg. }}}
\def\cis{{\text{cis }}}
\def\Cl{{\text{Cl }}}
\def\Div{{\text{Div }}}
%\def\Aut{{\text{Aut}}}
\DeclareMathOperator{\Aut}{Aut}
%\def\Out{{\text{Out}}}
\DeclareMathOperator{\Out}{Out}
\def\Gal{{\text{Gal}}}
\def\Ind{{\text{Ind}}}
\def\mod{{\mbox{mod }}}
\def\supp{{\mbox{supp }}}
\def\Ann{{\mbox{Ann }}}
\def\Spec{{\mbox{Spec }}}
\def\Specbf{{\textbf{Spec }}}
\def\Pic{{\text{Pic }}}
\def\Max{{\mbox{Max }}}
\def\mc#1{\mathcal{#1}}
\def\mf#1{\mathfrak{#1}}
\def\ol#1{\overline{#1}}
\def\ideles#1{{\mathbb A^{\times}_{#1}}}
\def\pairing#1#2{\langle #1, #2 \rangle}
\def\legendre#1#2{\left( \frac{#1}{#2} \right)}

\def\mapright#1{\smash{\mathop{\longrightarrow}\limits^{#1}}}
\def\mapdown#1{\Big\downarrow \rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}

\def\matrix#1#2#3#4{
    \left( \begin{array}{cc} #1&#2 \\ #3&#4 \end{array} \right)}
\def\threematrix#1#2#3#4#5#6#7#8#9{
    \left( \begin{array}{ccc} #1&#2&#3 \\ #4&#5&#6 \\ #7&#8&#9 \end{array} \right)}
\def\columnvector#1#2{
    \left ( \begin{array}{c} #1 \\ #2 \end{array} \right)}
\def\columnthreevector#1#2#3{
    \left ( \begin{array}{c} #1 \\ #2 \\ #3 \end{array} \right)}
\def\rowvector#1#2{
    \left ( \begin{array}{cc} #1 & #2 \end{array} \right)}
\def\rowthreevector#1#2#3{
    \left ( \begin{array}{ccc} #1 & #2 & #3 \end{array} \right)}
\def\blockmatrix#1#2#3#4{
    \left( \begin{array}{c|c} #1 & #2 \\ \hline #3 &
    #4 \end{array} \right)}
\def\Lie#1{{\mathfrak #1}}

\def\iff{\Longleftrightarrow}

\def\transpose {{\sp t}}
\def\half{{1 \over 2}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{predefinition}[theorem]{Definition}
\newenvironment{definition}{\begin{predefinition}\rm}{\end{predefinition}}
\newtheorem{preremark}[theorem]{Remark}
\newenvironment{remark}{\begin{preremark}\rm}{\end{preremark}}
\newtheorem{preconstruction}[theorem]{Construction}
\newenvironment{construction}{\begin{preconstruction}\rm}{\end{preconstruction}}
\newtheorem{prenotation}[theorem]{Notation}
\newenvironment{notation}{\begin{prenotation}\rm}{\end{prenotation}}
\newtheorem{preexample}[theorem]{Example}
\newenvironment{example}{\begin{preexample}\rm}{\end{preexample}}
\newtheorem{preclaim}[theorem]{Claim}
\newenvironment{claim}{\begin{preclaim}\rm}{\end{preclaim}}
\newtheorem{prequestion}[theorem]{Question}
\newenvironment{question}{\begin{prequestion}\rm}{\end{prequestion}}
%\newcommand {\thmref}[1] {Theorem \ref{#1}}                                                  
%\newcommand {\lemmaref}[1] {Lemma \ref{#1}}                                                  
%\newcommand {\propref}[1] {Proposition \ref{#1}}                                             
%\newcommand {\remref}[1] {Remark \ref{#1}}                                                   
%\newcommand {\conjref}[1] {Conjecture \ref{#1}}                                              
%\newcommand {\claimref}[1] {Claim \ref{#1}}                                                  
%\newcommand {\defnref}[1] {Definition \ref{#1}}                                              
%\newcommand {\corref}[1] {Corollary \ref{#1}}                                                
%\newcommand {\caseref}[1] {Case \ref{#1}}                                                    
%\newcommand {\exref}[1] {Example \ref{#1}}                                                   
%\newcommand {\exsref}[1] {Examples \ref{#1}}                                                 
%\newcommand {\eqnref}[1] {Equation \ref{#1}}

\newcommand{\bbmu}{\mu\hspace{-0.065in}\mu}
\newcommand{\bbalpha}{\alpha\hspace{-0.065in}\alpha} 

